Word Discovery in Visually Grounded, Self-Supervised Speech Models

We present a method for visually-grounded spoken term discovery. After training either a HuBERT or wav2vec2.0 model to associate spoken captions with natural images, we show that powerful word segmentation and clustering capability emerges within the model's self-attention heads. Our experiments reveal that this ability is not present to nearly the same extent in the base HuBERT and wav2vec2.0 models, suggesting that the visual grounding task is a crucial component of the word discovery capability we observe. We also evaluate our method on the Buckeye word segmentation and ZeroSpeech spoken term discovery tasks, where we perform on par with or better than currently published methods on several metrics. Code and model weights are available at https://github.com/jasonppy/word-discovery.

==> word_table.tex <==
\begin{table}[h]
    \caption{Codes are treated as word detectors ranked by the highest $F_1$ score among the words their are assigned to. Words that occur less than 10 times are not shown. \DHnote{hopefully we can keep at least part of this table, but it might end up taking too much space.}}
    \vspace{-6mm}
    \label{tab:detected_words}
    \begin{center}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{cccrrrr}
        \toprule
   Rank & Code &       Word &     $F_1$ &   Prec & Recall &   Occ\\
        \midrule
  2 &   74 &      trail & 100.00 & 100.00 & 100.00 &    34 \\
  3 & 1045 &    chewing & 100.00 & 100.00 & 100.00 &    18 \\
  4 & 3830 &     harbor & 100.00 & 100.00 & 100.00 &    19 \\
  8 &  211 &      smart & 100.00 & 100.00 & 100.00 &    22 \\
 11 & 3570 &  shirtless & 100.00 & 100.00 & 100.00 &    12 \\
 13 & 1082 &     garage & 100.00 & 100.00 & 100.00 &    19 \\
 16 & 3918 & locomotive & 100.00 & 100.00 & 100.00 &    20 \\
 24 & 2300 &       soup & 100.00 & 100.00 & 100.00 &    25 \\
 31 & 1367 &       dirt &  98.67 &  99.33 &  98.01 &   148 \\
 32 & 4052 &  christmas &  98.51 &  97.06 & 100.00 &    33 \\
 33 & 2331 &      boxes &  98.36 & 100.00 &  96.77 &    30 \\
 34 & 1931 &    hydrant &  98.17 &  97.92 &  98.43 &   188 \\
 35 & 4077 &     public &  98.00 &  98.00 &  98.00 &    49 \\
 36 & 1269 &      mouth &  97.90 &  97.22 &  98.59 &    70 \\
 37 & 1116 &      polar &  97.73 &  95.56 & 100.00 &    43 \\
 38 &  536 &  buildings &  97.65 &  99.05 &  96.30 &   104 \\
 39 &  505 &       wine &  97.51 &  96.08 &  98.99 &    98 \\
 40 & 2762 &     batter &  97.48 &  95.08 & 100.00 &    58 \\
 \multicolumn{7}{c}{$\cdots$} \\
180 & 3181 &      rural &  90.32 &  93.33 &  87.50 &    14 \\
181 & 1755 &      jeans &  90.32 &  87.50 &  93.33 &    14 \\
182 & 3492 &    carrots &  90.10 &  86.67 &  93.81 &    91 \\
183 & 3849 &      stack &  90.00 &  81.82 & 100.00 &    18 \\
186 & 2522 &      cakes &  90.00 &  90.00 &  90.00 &    18 \\
187 & 2264 &      apple &  89.92 &  96.67 &  84.06 &    58 \\
188 & 1089 &   distance &  89.86 &  83.78 &  96.88 &    31 \\
189 & 2276 &       team &  89.80 &  84.62 &  95.65 &    22 \\
190 & 1189 &   colorful &  89.74 &  97.22 &  83.33 &    70 \\
191 &  490 &      leash &  89.66 &  81.25 & 100.00 &    13 \\
192 & 1372 &   shopping &  89.66 &  81.25 & 100.00 &    13 \\
193 & 1972 &       eyes &  89.55 &  90.91 &  88.24 &    30 \\
194 & 1778 &        kid &  89.52 &  97.92 &  82.46 &    47 \\
195 &  653 &      tabby &  89.47 &  94.44 &  85.00 &    17 \\
196 & 2378 &       meal &  89.43 &  82.09 &  98.21 &    55 \\
197 &  934 &   commuter &  89.36 &  80.77 & 100.00 &    21 \\
198 & 1498 &    highway &  89.36 &  80.77 & 100.00 &    21 \\
199 & 1859 &     bottom &  89.36 &  91.30 &  87.50 &    21 \\
200 & 2856 &     screen &  89.31 &  84.52 &  94.67 &    71 \\
        \bottomrule
    \end{tabular}
    }
    \end{center}
\end{table}
